Person-job fit estimation from candidate profile and related recruitment history with co-attention neural networks

Existing online recruitment platforms depend on automatic ways of conducting the person-job fit, whose goal is matching appropriate job seekers with job positions. Intuitively, the previous successful recruitment records contain important information, which should be helpful for the current person-job fit. Existing studies on person-job fit, however, mainly focus on calculating the similarity between the candidate resumes and the job postings on the basis of their contents, without taking the recruiters' experience (i.e., historical successful recruitment records) into consideration. In this paper, we propose a novel neural network approach for person-job fit, which estimates person-job fit from candidate profile and related recruitment history with co-attention neural networks (named PJFCANN). Specifically, given a target resume-job post pair, PJFCANN generates local semantic representations through co-attention neural networks and global experience representations via graph neural networks. The final matching degree is calculated by combining these two representations. In this way, the historical successful recruitment records are introduced to enrich the features of resumes and job postings and strengthen the current matching process. Extensive experiments conducted on a large-scale recruitment dataset verify the effectiveness of PJFCANN compared with several state-of-the-art baselines. The codes are released at: https://github.com/CCIIPLab/PJFCANN.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> section/2_preliminaries.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   SECTION 2  %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Preliminary}
\label{sec:prelimi}

%
Typically, sequence labeling can be treated as a set of independent classification tasks,
which makes the optimal label for each member and then the global
best set of labels is chosen for the given sequence at once.
%select the globally best set of labels for 
%
Suppose we have a sequence ($\hat{x}$) composed of $n$ tokens, \ie $\hat{x}=[x_1, x_2, \ldots, x_n]^{\top}$,
%
we aim to assign a tag to each member
%
and output the corresponding globally best label sequence $\hat{y}=[y_1,y_2, \ldots, y_n]^{\top}$.
%
%However, accuracy is generally improved by making the optimal label for a given element dependent on the choices of nearby elements, using special algorithms to choose the globally best set of labels for the entire sequence at once.
%As an example of why finding the globally best label sequence might produce better results than labeling one item at a time, consider the part-of-speech tagging task just described. Frequently, many words are members of multiple parts of speech, and the correct label of such a word can often be deduced from the correct label of the word to the immediate left or right.
%
%the aim of sequence labeling is to assign a tag for each word and output the corresponding ground truth label sequence $\hat{y}=(y_1,y_2, \ldots, y_n)$.
%
Many neural models are proposed for
this task~\cite{Lample2016Neural,Ma2016End}.
%
By following the success of the state-of-the-art neural network architecture,
we briefly describe a \emph{Bi-LSTM-CRF} model for this task,
which often consists of three major stages:
%
%Following the recent state-of-the-art models for sequence labeling tasks ~\cite{Plank2016Multilingual,Lample2016Neural,Ma2016End}, we will use a Bi-directional LSTM-CRF model as our baseline. The model consists of mainly three stages:


\paratitle{Distributed Representation}, represents words in low dimensional real-valued dense vectors,
where each dimension represents a latent feature. Besides pre-trained word embeddings for the basic input, several studies~\cite{Santos2014Learning,Ma2016End,Lample2016Neural} also incorporate character-level representations for exploiting useful intra-word information (\eg prefix or suffix).
% such as prefix and suffix.


\paratitle{Context Encoder}, captures the context dependencies and learns contextual representations for tag decoding.
%
Traditional methods easily face the risk of gradient vanishing/exploding problem,
and thus several variants of RNNs, \eg LSTMs~\cite{hochreiter1997long},
are widely employed to be the context encoder architecture for different sequence labeling tasks,
owing to their promising performance on handling such problems.
%
%As promising performance on handling the gradient vanishing/exploding problem, variants (\ie LSTMs~\cite{hochreiter1997long}) of RNNs are widely employed to be the context encoder architecture for different sequence labeling tasks.
%
%gradient vanishing/exploding problem (handle/appear)
%%%
%LSTMs~\cite{Schuster1997Bidirectional} are variants of RNNs designed to cope with gradient vanishing/exploding problems and has become a widely-used context encoder architecture in sequence labeling tasks.
Therefore, here we briefly illustrate a special case of LSTM-CRF model, \ie \emph{Bi-directional} LSTM-CRF, which
incorporate past/future contexts from both directions (forward/backward) to generate the hidden states
of each word, and then jointly concatenate them to represent the \emph{global} information of the entire sequence.
%
%it is crucial to incorporate context from both directions
%
%generally generates forward/backward hidden states to model the past/future context information for each word, and then both two hidden states are concatenated to be as the \emph{global} information of the entire sequence.

However,
%
the sequential way to process the inputs of RNNs
might weaken the sensitivity of modeling discrete context dependencies,
%
since it recursively compose each word with its forward/backward hidden state that encodes the entire history/future information.
As such, the latent relationship between each pair of words is not well extracted, which is closely related to the final prediction task.
%
To this end, in this paper we propose a self-attentional context fusion layer
to better capture the relations among tokens and help to model discrete context dependencies,
via incorporating the complementary context information at different layers
in our proposed neural architecture. We will detail it in the following
sections, respectively.


\paratitle{Tag Decoder},
%
employs a CRF layer to produce a sequence of tags corresponding to the input sequence.
%To make the optimal label for each element of a given sequence,
Typically, the correct label to each element of a given sequence
often depends on the choices of nearby elements.
%
As such, the correlations between labels of adjacent neighborhoods are usually
considered for jointly decoding the best chain of labels for the entire sequence.
%the correct label of such member is often depended on the choices of nearby elements,
% and it is thus beneficial to consider the correlations between labels of adjacent neighborhoods, and then jointly decode the best chain of labels for the entire sequence.
%
%For a sequence labeling task, it is beneficial to consider the correlations between labels in neighborhoods and jointly decode the best chain of labels for a given sequence.
%
Additionally, CRF model has been proven~\cite{lafferty2001conditional} to be powerful
in learning the strong dependencies across output labels,
%
thus it is usually employed to make the optimal label for each element of the input sequence.
%
Specifically,
%Conditional random field (CRF)~\cite{lafferty2001conditional} has been included in most top-performing models to learn the strong dependencies across output labels and model label sequence jointly.
%
let $\matrix{Z} = [\hat{z}_{1},\hat{z}_{2}, \ldots,\hat{z}_{n}]^{\top}$
be the output of context encoder of the given
%training instance
sequence $\hat{x}$,
%
and thus the probability $\Pr(\hat{y}|\hat{x})$ of generating the whole label sequence $\hat{y}$ with regard to $\matrix{Z}$
is calculated by CRF model~\cite{Liu2017Empower},
%
%$(x_i,y_i)$, we suppose the output of context encoder is $\matrix{Z}_i = [\hat{z}_{i,1},\hat{z}_{i,2}, \ldots,\hat{z}_{i,n}]^{\top}$. CRF models describe the probability $\Pr(\hat{y}|x_i)$ of generating the whole label sequence $y_i\in\hat{y}$ with regard to $Z$, and the probability is defined as follows:
%
\begin{equation}
  \Pr(\hat{y}|\hat{x}) = \frac{\prod_{j=1}^{n}\phi(y_{j-1},y_j,\hat{z}_j)}
{\sum_{y^{'}\in{\matrix{Y}(\matrix{Z})}}\prod_{j=1}^n\phi(y^{'}_{j-1},y^{'}_j,\hat{z}_j)},
\end{equation}

\begin{equation}
	\phi(y_{j-1},y_j,\hat{z}_j)\!=\!\exp(\matrix{W}_{y_{j-1},y_{j}}\hat{z}_j + b_{y_{j-1},y_j}),
\end{equation}
where $\matrix{Y}(\matrix{Z})$ is the set of possible label sequences for $\matrix{Z}$;
%
%
$\matrix{W}_{y_{j-1},y_{j}}$ and  $b_{y_{j-1},y_j}$
indicate the weighted matrix and bias parameters corresponding to the label pair $(y_{j-1},y_j)$, respectively.
%
Then, we employ a likelihood function $\mathcal{L}$
to minimize the negative \emph{log} probability of the golden tag sequence for training,
%where the loss of the function is defined as $\mathcal{L}$:
%
\begin{equation}
\mathcal{L} = -\sum_{\hat{x}\in \mathcal{X};\hat{y}\in \mathcal{Y}}\log p(\hat{y}|\hat{x}),
\end{equation}
where $\mathcal{X}$ denotes the set of training instances, and $\mathcal{Y}$ indicates the corresponding
tag set.




%\begin{itemize}
%\item $\textbf{Distributed Representation}$, represents words in low dimensional real-valued dense vectors;
%\item $\textbf{Context Encoder}$, uses a bi-directional LSTM framework to learn the context features from input representations;
%\item $\textbf{Tag Decoder}$, typically employs a CRF layer to produce a sequence of tags corresponding to the input sequence.
%\end{itemize}


%%%%%%%%%%%%%%
\eat{
\subsection{Distributed Representation}
Distributed representation represents words in low dimensional real-valued dense vectors where each dimension represents a latent feature~\cite{li2018survey}. Besides pre-trained word embeddings for the basic input, several studies~\cite{Santos2014Learning,Ma2016End,Lample2016Neural} incorporate character-level representations for exploiting useful intra-word information such as prefix and suffix.}


%%%%%%%%%%%%%%
\eat{
\subsection{Context Encoder}
\label{ContextEncoder}
The aim of context encoder is to capture the context dependencies and then extract word contextual representations for tag decoding. LSTMs~\cite{Schuster1997Bidirectional} are variants of RNNs designed to cope with gradient vanishing/exploding problems and has become a widely-used context encoder architecture in sequence labeling tasks. \emph{Bi-directional LSTM-CRF} model adopts a LSTM in both directions, generating a forward hidden state and a backward hidden state for each word to extract past and future context information. Then the two hidden states are concatenated to give global information of the whole sequence.

However, we argue that the sequential way to process the inputs of RNNs might weaken the sensitivity of models to context dependencies. Because it recursively compose each word with its forward/backward hidden state that encodes the entire history/future information, and the latent relationship among words is not well extracted to some extent, which is closely related to the final prediction task.
%${w_i}$
%\begin{math}  ${\small \stackrel{\rightarrow}{h_i}}$  $\stackrel{\leftarrow}{h_i}$
%{h_i = [\stackrel{\rightarrow}{h_i},\stackrel{\leftarrow}{h_i}]}.
%\end{math}
}
%%%%%%%%%%%%%%
\eat{
\subsection{Tag Decoder}
%To make the optimal label for each element of a given sequence,
Typically, the correct label of each member of a given sequence
is often depended on the choices of nearby elements.
%
As such, the correlations between labels of adjacent neighborhoods are usually
considered for jointly decoding the best chain of labels for the entire sequence.
%the correct label of such member is often depended on the choices of nearby elements,
% and it is thus beneficial to consider the correlations between labels of adjacent neighborhoods, and then jointly decode the best chain of labels for the entire sequence.
%
%For a sequence labeling task, it is beneficial to consider the correlations between labels in neighborhoods and jointly decode the best chain of labels for a given sequence.
%
Additionally, CRF model has been proven~\cite{lafferty2001conditional} to be powerful
in learning the strong dependencies across output labels and model labeling sequence jointly.
%
Therefore, here we employ a CRF model to make the optimal label for each element of the input sequence.
%
Specifically,
%Conditional random field (CRF)~\cite{lafferty2001conditional} has been included in most top-performing models to learn the strong dependencies across output labels and model label sequence jointly.
%
let $\matrix{Z} = [\hat{z}_{1},\hat{z}_{2}, \ldots,\hat{z}_{n}]^{\top}$
be the output of context encoder of the given training instance $\hat{x}$,
%
and thus the probability $\Pr(\hat{y}|\hat{x})$ of generating the whole label sequence $y_i\in\hat{y}$ with regard to $\matrix{Z}$
is calculated by CRF model~\cite{Liu2017Empower},
%
%$(x_i,y_i)$, we suppose the output of context encoder is $\matrix{Z}_i = [\hat{z}_{i,1},\hat{z}_{i,2}, \ldots,\hat{z}_{i,n}]^{\top}$. CRF models describe the probability $\Pr(\hat{y}|x_i)$ of generating the whole label sequence $y_i\in\hat{y}$ with regard to $Z$, and the probability is defined as follows:
%
\begin{equation}
  \Pr(\hat{y}|\hat{x}) = \frac{\prod_{j=1}^{n}\phi(y_{j-1},y_j,\hat{z}_j)}
{\sum_{y^{'}\in{\matrix{Y}(\matrix{Z})}}\prod_{j=1}^n\phi(y^{'}_{j-1},y^{'}_j,\hat{z}_j)},
\end{equation}
where $\matrix{Y}(\matrix{Z})$ is the set of possible label sequences for $\matrix{Z}$;
%
\begin{math}
  \phi(y_{j-1},y_j,\hat{z}_j)\!=\!\exp(\matrix{W}_{y_{j-1},y_{j}}\hat{z}_j + b_{y_{j-1},y_j}),
\end{math}
%
$\matrix{W}_{y_{j-1},y_{j}}$ and  $b_{y_{j-1},y_j}$
indicate the weighted matrix and bias parameters corresponding to the label pair $(y_{j-1},y_j)$, respectively.
%
Then, we employ a likelihood function $\mathcal{L}$
to minimize the negative \emph{log} probability of the golden tag sequence for training,
%where the loss of the function is defined as $\mathcal{L}$:
%
\begin{equation}
\mathcal{L} = -\sum_{\hat{x}\in \mathcal{X};\hat{y}\in \mathcal{Y}}\log p(\hat{y}|\hat{x}),
\end{equation}
where $\mathcal{X}$ denotes the set of training instances, and $\mathcal{Y}$ indicates the corresponding
tag set.}

